Molecular docking via quantum approximate optimization algorithm

Molecular docking plays a pivotal role in drug discovery and precision medicine, enabling us to understand protein functions and advance novel therapeutics. Here, we introduce a potential alternative solution to this problem, the digitized-counterdiabatic quantum approximate optimization algorithm (DC-QAOA), which utilizes counterdiabatic driving and QAOA on a quantum computer. Our method was applied to analyze diverse biological systems, including the SARS-CoV-2 Mpro complex with PM-2-020B, the DPP-4 complex with piperidine fused imidazopyridine 34, and the HIV-1 gp120 complex with JP-III-048. The DC-QAOA exhibits superior performance, providing more accurate and biologically relevant docking results, especially for larger molecular docking problems. Moreover, QAOA-based algorithms demonstrate enhanced hardware compatibility in the noisy intermediate-scale quantum era, indicating their potential for efficient implementation under practical docking scenarios. Our findings underscore quantum computing's potential in drug discovery and offer valuable insights for optimizing protein-ligand docking processes.

==> name.tex <==

In the conventional QAOA frameworks, achieving a near-optimal solution often necessitates a substantial parameter \( p \). This requirement exacerbates the complexity of implementing the unitary operator \( U(\boldsymbol{\gamma},\boldsymbol{\beta}) \), leading to inefficiencies that pose significant challenges for Near-term Intermediate-Scale Quantum (NISQ) devices. To alleviate this issue, the Digitized-Counterdiabatic QAOA (DC-QAOA) was proposed, as detailed in \cite{chandarana2022digitized}. This methodology integrates a counterdiabatic (\(\mathrm{CD}\)) driving term into conventional QAOA algorithms by introducing an additional variational parameter at each stage, thereby transforming \( U(\boldsymbol{\gamma}, \boldsymbol{\beta}) \) into \( U(\boldsymbol{\gamma}, \boldsymbol{\beta}, \boldsymbol{\alpha}) \) and \( F(\boldsymbol{\gamma}, \boldsymbol{\beta}) \) into \( F(\boldsymbol{\gamma}, \boldsymbol{\beta}, \boldsymbol{\alpha}) \) [Refer to FIG.~\ref{fig:process}]. Empirical evidence suggests that these supplementary parameters substantially diminish the requisite value of \( p \) to attain a near-optimal trial state \cite{chandarana2022digitized}.

The integration of the CD driving term into the problem Hamiltonian can be quantified as emanating from the concept of shortcuts to adiabaticity~\cite{chen2010shortcut,chen2010fast,hegade2021shortcuts}. This principle is pivotal for mitigating nonadiabatic transitions and expediting quantum adiabatic processes~\cite{del2012assisted,demirplak2005assisted,demirplak2003adiabatic,berry2009transitionless}, with notable applications in quantum state preparation tasks~\cite{yao2021reinforcement}.

In this study, we adhere to the methodology delineated in \cite{chandarana2022digitized} and adopt the nested commutator framework of the adiabatic gauge potential as introduced by Claeys et al.~\cite{claeys2019floquet}, to construct a pool of CD operators, expressed as
\begin{equation}
    A_\lambda^{(l)}=i \sum_{k=1}^l \alpha_k(t) \underbrace{\left[H_a,\left[H_a, \ldots\left[H_a, \right.\right.\right.}_{2 k-1}\partial_\lambda H_a]]] .
\end{equation}
In this approach, we confine our consideration to the second order in the expansion of the nested commutator, i.e., \( l=2 \). The operator pool \( A \) is defined as \( \{\sigma^y, \sigma^z \sigma^y, \sigma^y \sigma^z, \sigma^x \sigma^y, \sigma^y \sigma^x\} \), encompassing solely local and two-body interactions. It is imperative to note that the selection of this operator pool is contingent on the problem Hamiltonian, and may include other operators pertinent to specific problems.

In the context of the Ising model, a pivotal study has outlined a method for selecting counterdiabatic (CD) terms under varying conditions \cite{chandarana2022digitized}. This includes the formulation of the Hamiltonian for the one-dimensional Ising spin model, represented as \( H_{\text{prob}}(\sigma) = -\sum_{(i,j)} J_{ij}\sigma^z_i \sigma^z_j - \sum_{i} h_i\sigma^z_i - \sum_{i} k_i\sigma^x_i \), where \(\sigma^d_i\) denotes the Pauli matrices at each site and \((i, j)\) corresponds to nearest-neighbor interactions with strength \(J_{ij}\). Within this framework, two distinct scenarios emerge: The Linear Ferromagnetic Ising Model (LFIM), where the condition \(k_i = 0\) is met and the CD driving term is given as \(A_t = \sum_{i} \sigma^y_i\), and the Transverse-Field Ising Model (TFIM), characterized by \(h_i = 0\), with the CD driving term expressed as \(A_t = \sum_{i} \sigma^z_i \sigma^z_{i+1}\).

The unitary operator symbolizing the CD component of the circuit is delineated as
\begin{equation}
U_{\text{CD}}(\alpha) = \prod_{j=1}^{L} \exp [-i\alpha A_j^q]
\end{equation}
where \( A_j^q \) denotes the corresponding \( q \)-local CD operator selected from the CD pool \( A \). For instance, if \( q = 1 \), then \( A_j^1 = \{A_{j}\}_{j} \), and for \( q = 2 \), \( A_j^2 = \{A_{j,j+1}\}_{j} \). 

In the context of the Hamiltonian \( H_C \) for the Minimum Vertex Weight Clique Problem (MVWCP), our model aligns with the LFIM, hence our CD driving term is \(A_t = \sum_{i} \sigma^y_i\). 

To evaluate the resource requisites, both classical and quantum, it is imperative to examine two critical aspects of these methods. For systems with nearest-neighbor interactions, the increase in circuit depth per layer upon adding a CD term is constant, dependent on the selected CD term. The circuit depth is quantifiable as \( d \times p \), with the inclusion of the CD driving escalating it to \( (d + d_{\text{cd}}) \times p \), where \( d_{\text{cd}} \) signifies the increment in depth per layer. For the LFIM, the CD term \( \sigma_y \) results in \( d_{\text{cd}} = 1 \), whereas for the TFIM, \( d_{\text{cd}} = 4 \) for \( \sigma_z\sigma_y \). Conversely, the expansion in parameter space due to the CD term consistently alters from \( 2p \) to \( 3p \), rendering the DC-QAOA particularly beneficial for low \( p \) values. In the realm of large \( p \), the efficacy of QAOA and DC-QAOA converge for a fixed system size.


The Quantum Approximate Optimization Algorithm (QAOA) is designed to address combinatorial optimization challenges, employing adiabatic evolution guided by a time-dependent Hamiltonian \( H_a(t) = [1 - \lambda(t)] H_{\text{M}} + \lambda(t) H_{\text{C}} \), where $\lambda(t)$ transitions the system from \( H_{\text{M}} \) to \( H_{\text{C}} \) over time \( t \). The adiabatic theorem ensures that the system's ground state evolves from \( H_{\text{M}} \) to that of \( H_{\text{C}} \), encoding the solution.

QAOA approximates this evolution using alternating unitary operations \( U_m(\beta_j) = \exp(-i \beta_j H_{\text{M}}) \) and \( U_c(\gamma_j) = \exp(-i \gamma_j H_{\text{C}}) \), defined by parameters \( \beta_j \) and \( \gamma_j \), within a limited iteration count \( p \):
\begin{equation}
   U(\boldsymbol{\gamma}, \boldsymbol{\beta}) = \ldots U_m(\beta_1) U_c(\gamma_1).
\end{equation}
The QAOA ansatz depth, characterized by the \( 2p \) parameter space \( (\boldsymbol{\gamma}, \boldsymbol{\beta}) \), represents the sequential applications of \( U_c \) and \( U_m \).

The goal is to maximize the expected value \( F_p(\boldsymbol{\gamma}, \boldsymbol{\beta}) = \langle \boldsymbol{\gamma}, \boldsymbol{\beta} | H_C | \boldsymbol{\gamma}, \boldsymbol{\beta} \rangle \) by tuning \( \boldsymbol{\gamma}, \boldsymbol{\beta} \) to achieve
\begin{equation}
M_p = \max_{\boldsymbol{\gamma}, \boldsymbol{\beta}} F_p(\boldsymbol{\gamma}, \boldsymbol{\beta}),
\end{equation}
representing the approximate optimal solution for a given \( p \).

In standard QAOA, a high \( p \) value is often needed for near-optimal solutions, complicating the implementation of \( U(\boldsymbol{\gamma},\boldsymbol{\beta}) \) and challenging NISQ devices. DC-QAOA, introduced in \cite{chandarana2022digitized}, incorporates a counterdiabatic (\(\mathrm{CD}\)) term, adding an extra variational parameter and transforming \( U(\boldsymbol{\gamma}, \boldsymbol{\beta}) \) into \( U(\boldsymbol{\gamma}, \boldsymbol{\beta}, \boldsymbol{\alpha}) \), significantly reducing the required \( p \).

The CD driving term is integrated based on shortcuts to adiabaticity principles. By employing the nested commutator methodology for the adiabatic gauge potential, we define a set of CD operators \( A_\lambda^{(l)} \) for local and two-body interactions, tailored to the problem Hamiltonian.

For the Ising model, CD term selection varies. The Hamiltonian for the one-dimensional Ising spin model is given as \( H_{\text{prob}}(\sigma) = -\sum_{(i,j)} J_{ij}\sigma^z_i \sigma^z_j - \sum_{i} h_i\sigma^z_i - \sum_{i} k_i\sigma^x_i \). For the LFIM (\( k_i = 0 \)), the CD driving term is \( A_t = \sum_{i} \sigma^y_i \), and for the TFIM (\( h_i = 0 \)), it is \( A_t = \sum_{i} \sigma^z_i \sigma^z_{i+1} \).

The CD component of the quantum circuit is captured by
\begin{equation}
U_{\text{CD}}(\alpha) = \prod_{j=1}^{L} \exp [-i\alpha A_j^q],
\end{equation}
where \( A_j^q \) is the \( q \)-local CD operator from \( A \). The circuit depth increment per layer due to the CD term is constant, resulting in an overall depth of \( (d + d_{\text{cd}}) \times p \), with \( d_{\text{cd}} \) depending on the CD term.

{The general workflow of protein-ligands docking via QAOA algorithms is illustrated in FIG.~\ref{fig:process}.}


The Quantum Approximate Optimization Algorithm (QAOA) is a quantum algorithm recently introduced to tackle the combinatorial optimization problems. It utilizes the concept of adiabatic evolution, guided by a time-dependent Hamiltonian $H_a(t)$, articulated as:
\begin{equation}
H_a(t) = [1 - \lambda(t)] H_{\text{M}} + \lambda(t) H_{\text{C}},
\end{equation}
where $\lambda(t) \in [0,1]$ denotes the annealing protocol across the time interval $t \in [0, T]$.
Practically, the problem at hand is encoded into the ground state of the Hamiltonian $H_{\text{C}}$ (typically a state challenging to construct), commencing from a Hamiltonian $H_{\text{M}}$ with a readily preparable ground state, and gradually transitioning to Hamiltonian $H_{\text{C}}$. According to the adiabatic theorem, if the adiabatic condition is fulfilled, the ground state of a quantum system will progressively transition from the ground state of $H_{\text{M}}$ to that of $H_{\text{C}}$, thereby facilitating the extraction of the problem's solution through decoding. 

QAOA, as an approximation methodology, simulates the original evolution through alternating unitary operations $U_m(\beta_j) = \exp(-i \beta_j H_{\text{M}})$ and $U_c(\gamma_j) = \exp(-i \gamma_j H_{\text{C}})$, characterized by parameters $\beta_j$ and $\gamma_j$, within a limited iteration count $p$ but with adjustable temporal evolution parameters, as delineated below:
\begin{equation}
   \begin{aligned}
U(\boldsymbol{\gamma}, \boldsymbol{\beta}) = & U_m\left(\beta_p\right) U_c\left(\gamma_p\right) U_m\left(\beta_{p-1}\right) U_c\left(\gamma_{p-1}\right) \ldots \\
& \ldots U_m\left(\beta_1\right) U_c\left(\gamma_1\right),
\end{aligned}
\end{equation}

It is observed that the integer \( p \) signifies the number of sequential applications of \( U_c \) and \( U_m \), implying that \( U_c \) and \( U_m \) are alternately applied \( p \) times to the initial state. The circuit $U(\boldsymbol{\gamma}, \boldsymbol{\beta})$ is also referred to as the QAOA ansatz, with the ansatz depth characterized by the $2p$ parameter space $(\boldsymbol{\gamma}, \boldsymbol{\beta})$, where $\boldsymbol{\beta} = (\beta_p, \beta_{p-1}, \ldots, \beta_1)$ and $\boldsymbol{\gamma} = (\gamma_p, \gamma_{p-1}, \ldots, \gamma_1)$.

The expected value of the Hamiltonian \( H_C \) in the quantum state is denoted by \( F_p(\boldsymbol{\gamma}, \boldsymbol{\beta}) \):
\begin{equation}
F_p(\boldsymbol{\gamma}, \boldsymbol{\beta}) = \langle \boldsymbol{\gamma}, \boldsymbol{\beta} | H_C | \boldsymbol{\gamma}, \boldsymbol{\beta} \rangle.
\end{equation}
Specifically, the quantum aspect entails evaluating the cost function $F_p(\boldsymbol{\gamma}, \boldsymbol{\beta})$, while the classical part involves determining the optimal parameter set $\left(\boldsymbol{\gamma}^*, \boldsymbol{\beta}^*\right)$ that maximizes $F_p$. 

By modulating the parameters \( \boldsymbol{\gamma}, \boldsymbol{\beta} \), we achieve
\begin{equation}
M_p = \max_{\boldsymbol{\gamma}, \boldsymbol{\beta}} F_p(\boldsymbol{\gamma}, \boldsymbol{\beta})
\end{equation}
as the approximate optimal solution for a given layer count \( p \). It is noteworthy that the search space enabled by \( p \) layers of \( U_c \) and \( U_m \) surpasses that of \( p - 1 \) layers.

In the conventional QAOA frameworks, achieving a near-optimal solution often necessitates a substantial parameter \( p \). This requirement exacerbates the complexity of implementing the unitary operator \( U(\boldsymbol{\gamma},\boldsymbol{\beta}) \), leading to inefficiencies that pose significant challenges for NISQ devices. The Digitized-Counterdiabatic QAOA (DC-QAOA), as expounded in \cite{chandarana2022digitized}, addresses this by embedding a counterdiabatic (\(\mathrm{CD}\)) term in standard QAOA, introducing an extra variational parameter at each iteration, thereby transforming \( U(\boldsymbol{\gamma}, \boldsymbol{\beta}) \) into \( U(\boldsymbol{\gamma}, \boldsymbol{\beta}, \boldsymbol{\alpha}) \) and \( F(\boldsymbol{\gamma}, \boldsymbol{\beta}) \) into \( F(\boldsymbol{\gamma}, \boldsymbol{\beta}, \boldsymbol{\alpha}) \), as depicted in FIG.~\ref{fig:process}. Empirical evidence suggests that these supplementary parameters substantially diminish the requisite value of \( p \) to attain a near-optimal trial state \cite{chandarana2022digitized}.

The integration of the CD driving term, based on shortcuts to adiabaticity principles~\cite{chen2010shortcut,chen2010fast,hegade2021shortcuts}, mitigates nonadiabatic transitions and accelerates quantum processes, as noted in studies such as ~\cite{del2012assisted,demirplak2005assisted,demirplak2003adiabatic,berry2009transitionless}, with notable applications in quantum state preparation tasks~\cite{yao2021reinforcement}. Utilizing the nested commutator methodology for the adiabatic gauge potential~\cite{claeys2019floquet}, we define a specific set of CD operators \( A_\lambda^{(l)} \) up to second order (\( l=2 \)), comprising local and two-body interactions. The choice of operators is tailored to the problem Hamiltonian and can include variants based on the system's requirements.

In the context of the Ising model, a pivotal study has outlined a method for selecting counterdiabatic (CD) terms under varying conditions \cite{chandarana2022digitized}. This includes the formulation of the Hamiltonian for the one-dimensional Ising spin model, represented as \( H_{\text{prob}}(\sigma) = -\sum_{(i,j)} J_{ij}\sigma^z_i \sigma^z_j - \sum_{i} h_i\sigma^z_i - \sum_{i} k_i\sigma^x_i \), where \(\sigma^d_i\) denotes the Pauli matrices at each site and \((i, j)\) corresponds to nearest-neighbor interactions with strength \(J_{ij}\). Within this framework, two distinct scenarios emerge: The Linear Ferromagnetic Ising Model (LFIM), where the condition \(k_i = 0\) is met and the CD driving term is given as \(A_t = \sum_{i} \sigma^y_i\), and the Transverse-Field Ising Model (TFIM), characterized by \(h_i = 0\), with the CD driving term expressed as \(A_t = \sum_{i} \sigma^z_i \sigma^z_{i+1}\). In the context of the Hamiltonian \( H_C \) for the Minimum Vertex Weight Clique Problem (MVWCP) in Eq. (\ref{eq:Hamiltonian}), our model aligns with the LFIM, hence our CD driving term is \(A_t = \sum_{i} \sigma^y_i\). 

The CD component in the quantum circuit is represented by the unitary operator
\begin{equation}
U_{\text{CD}}(\alpha) = \prod_{j=1}^{L} \exp [-i\alpha A_j^q]
\end{equation}
where \( A_j^q \) is the \( q \)-local CD operator from the set \( A \). 

In assessing resource implications, the circuit depth increment per layer is crucial. The addition of a CD term results in a constant depth increase, dependent on the CD term, with the overall depth being \( (d + d_{\text{cd}}) \times p \). For the LFIM, this increase is modest (\( d_{\text{cd}} = 1 \)), whereas for the TFIM, it is more significant (\( d_{\text{cd}} = 4 \)). The parameter space expansion from \( 2p \) to \( 3p \) through the CD term renders DC-QAOA advantageous for lower \( p \) values, with its efficacy converging with traditional QAOA at high \( p \) values for a given system size.

{We summarize the general processing flow of the protein-ligands docking via QAOA algorithms, as shown in FIG.~\ref{fig:process}.}


In the domain of protein-ligand docking, the significance attributed to individual atoms is heterogeneously distributed. Our research predominantly concentrates on pharmacophores — distinct atomic conglomerates critical in mediating a molecule's pharmacological and biological interactions. These pharmacophores encompass entities bearing either negative or positive charges, hydrogen-bond donors or acceptors, hydrophobic elements, and aromatic rings. To efficaciously delineate the In order to precisely depict the spatial interrelationships among these pharmacophoric points in proteins (ligands), we have developed a labeled distance graph refer to the initial segment of FIG.~\ref{fig:process}. For each protein or ligand molecule under examination, pharmacophore points engaged in binding interactions are heuristically selected to constitute the graph's vertices, each annotated based on its characteristic type. Interconnecting these vertices, edges are instituted, with their weights determined by the Euclidean distances between the respective pharmacophoric points. {This graphical representation enables the observation of spatial correlations between the docking points of interest on the protein or ligand.}

Upon selecting the protein or ligand for investigation, the subsequent phase involves constructing a Binding Interaction Graph (BIG), intended to model the docking relationship, thereby elucidating potential interplays among pharmacophoric points, as demonstrated in the latter segment of FIG.~\ref{fig:process}. This graph is generated through the amalgamation of the labeled distance graphs pertaining to both the ligand and the protein, culminating in a comprehensive representation that encapsulates all theoretical interaction pairings. The cumulative vertex count in this graph is expressed as 
$nm$, where $n$ and $m$ represent the number of vertices in the ligand and protein binding site graphs, respectively. This framework facilitates the selection of any one of the 
$n$ points on the ligand and any one of the $m$ points on the protein to instantiate a vertex within the Binding Interaction Graph.


In the domain of protein-ligand docking, it is axiomatic that the significance of atoms is not homogeneously distributed. Our investigation primarily concentrates on pharmacophores — distinct atomic configurations quintessential in determining a molecule's pharmacological and biological interactions. These pharmacophores encompass entities bearing either negative or positive charges, entities functioning as hydrogen-bond donors or acceptors, hydrophobic elements, and aromatic rings. Given the constraints of our current quantum computational resources, we are necessitated to either focus on a subset of salient pharmacophores or to heuristically select pharmacophore points engaged in subsequent binding interactions. To delineate the geometric relationships of pharmacophores in proteins(ligands), we construct a Labeled Distance Graph (LDG), as depicted in the initial segment of FIG.~\ref{fig:process}. In constructing LDG for proteins(ligands), the vertices are the selecting  pharmacophore points, each vertex being appropriately labeled to reflect its typology. Interconnecting these vertices are edges, the weights of which are assigned based on the Euclidean distances between the respective pharmacophore points. This graphical representation enables the elucidation of spatial relationships amongst pharmacophores, particularly focusing on the docking points of interest on the protein or ligand under study.

Upon the selection and construction of the Ligand-Dependent Graph (LDG) for either the protein or ligand, the subsequent phase entails the formation of a Binding Interaction Graph (BIG). This graph is pivotal in depicting the docking correlation, thereby facilitating the illustration of prospective interactions among pharmacophore points, as delineated in the second segment of FIG.~\ref{fig:process}. The BIG is synthesized via a comprehensive integration of the LDGs of both the ligand and the protein. This integration yields an extensive representation, capturing all theoretically plausible interaction pairings, herein referred to as "connects". The aggregate vertex count in the BIG is signified by $nm$, where $n$ and $m$ denote the number of vertices in the LDG of the ligand and the protein, respectively. This notation permits the selection of any vertex from the set of $n$ vertices on the ligand and any from the set of $m$ vertices on the protein, thus forming a vertex within the BIG. The edges in BIG indicate the simultaneous existence of two connects, leading to the inference that a clique signifies the coexistence of all vertices within the clique, representing potential binding postures through sets of contacts.

In the BIG, each edge symbolizes a pair of vertices, implying that both vertices represented by the edge can concurrently exist within a docking posture. This denotes that every vertex within a group in the BIG can coexist, collectively delineating a feasible docking posture. Moreover, the group with the maximal weight in the BIG is indicative of the most probable docking posture among all possible configurations.

Each edge in the BIG represents two vertices on the edge that can exist in a docking posture at the same time. This means that all the vertices contained in a clique in the BIG can coexist, representing a viable docking posture. And the MVWCP in the BIG represents the most likely docking posture of all the docking posture.



Suppose we have obtained the BIG for a specific molecular docking problem. Consider the undirected graph $\text{BIG} =(V, E)$, where $V$ and $E$ represent the vertex and edge sets, respectively. Each vertex is assigned a positive weight $w_i$, which denotes the pharmacophore potential in molecular docking problem. The MVWCP can be modeled as a binary quadratic programming (BQP) problem as follows~\cite{wang2016solving}:
\begin{equation}
\begin{aligned}
\operatorname{maximize} \quad & \sum_{i=1}^N w_i x_i+\sum_{i=1}^N \sum_{j=1, j \neq i}^N w_{i j} x_i x_j \\
\text{subject to:} \quad & x_i \in\{0,1\}, i \in\{1, \ldots, N\}
\end{aligned}
\label{eq:mvwc2}
\end{equation}
where $N=|V|$ represents the size of the problem, which is the number of qubits used to solve it, and $x_i$ represents the binary variable associated with vertex $v_i$. We have 
$w_{i j}=P$ if $\left\{v_i, v_j\right\} \in \bar{E}$ and 0 otherwise, where $\bar{E}$ is the set of edge of complementary graph $\bar{G}$ and $P$ is a designated negative penalty scalar. This formulation is one of many nonlinear reformulations of the MVWCP and has been studied in previous work like \cite{horst2000introduction}. The quadratic function yields an equivalent objective value to the linear form when all penalty terms are set to 0, signifying the fulfillment of all constraints. According to Eq. (\ref{eq:mvwc2}), any violated constraint, i.e., for each $\left\{v_i, v_j\right\} \in \bar{E}$, in a solution will add a penalty value 2P to the objective value. Theoretically, the larger the absolute value of the penalty function $|P|$, the easier it is to get a more correct result, because the penalty term prevents the generation of edges that should not occur. In classical calculations, we can often set $P \geq −1000 \sum_{i=1}^{N} w_i$. However, in the case of quantum computer simulations, we found that the P value could not be increased arbitrarily, which would lead to inaccurate results. This is because if P is very large, the coefficient of $w_i$ will be very small after normalization, and it is not easy for the QAOA algorithm to search for the optimal solution. We will analyze these situations in detail in following examples.
